A Faraday Rotation Study of the Stellar Bubble and HII Region Associated with the W4 Complex

We utilized the Very Large Array to make multifrequency polarization measurements of 20 radio sources viewed through the IC 1805 HII region and "Superbubble", as well as in the immediate vicinity. The measurements at frequencies between 4.33 and 7.76 GHz yield Faraday rotation measures along 27 lines of sight to these sources (some sources have more than one component). The Faraday rotation measures (RM) are used to probe the plasma structure of the IC 1805 HII region and to test the degree to which the Galactic magnetic field is heavily modified (amplified) by the dynamics of the HII region. We find that similar to the Rosette Nebula (Savage et al. 2013, Costa et al. 2016) and the Cygnus OB1 association (Whiting et al. 2009), IC 1805 constitutes a "Faraday rotation anomaly", or a region of increased RM relative to the general Galactic background value. Although the RM observed on lines of sight through the region vary substantially, the |RM| due to the nebula is commonly 600 -- 800 rad m^-2. In spite of this, the observed RMs are not as large as simple, analytic models of magnetic field amplification in HII regions might indicate. This suggests that the Galactic field is not increased by a substantial factor within the ionized gas in an HII region. We also find that with one exception, the sign of the RM for all sources is that expected for the polarity of the Galactic field in this direction. The same behavior was found for the Rosette Nebula, and qualitatively indicates that turbulent fluctuations in the Galactic field on spatial scales of $\sim 10$ pc are smaller than the mean Galactic field. Finally, our results show intriguing indications that some of the largest values of |RM| occur for lines of sight that pass outside the fully ionized shell of the IC 1805 HII region, but pass through the Photodissociation Region (PDR) associated with IC 1805.

==> arvix submission final/defs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       defs.tex
% 
%       Thesis Definitions
%      
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%\newcommand{\THESISTITLE}{...TBA...}
%%
\newcommand{\bext}{\textbf{B}$_{\textrm{ext}}$}
\newcommand{\mhii}{\textrm{H}\,\textsc{ii}}
\newcommand{\mPhii}{P^{\textrm{H}\,\textsc{ii}}_{\textrm{th}}}
\newcommand{\Phii}{$P^{\textrm{H}\,\textsc{ii}}_{\textrm{th}}$}
\newcommand{\mPpdr}{P^{\textrm{PDR}}_{\textrm{th}}}
\newcommand{\Ppdr}{$P^{\textrm{PDR}}_{\textrm{th}}$}

\newcommand{\VLASS}{VLA Sky Survey (VLASS)}
\newcommand{\VLITE}{VLA Low-band Ionosphere and Transient Experiment (VLITE)}
\newcommand{\CGPS}{Canadian Galactic Plane Survey (CGPS)}
\newcommand{\NRAO}{National Radio Astronomy Observatory}
\newcommand{\CASAfootnote}{\footnotesize{See the NRAO Jansky VLA tutorial ``EVLA Continuum Tutorial 3C391'' (http$://$casaguides.nrao.edu$/$index.php$?$title$=$EVLA$_{-}$Continuum$_{-}$Tutorial$_{-}$3C391)}}
\newcommand{\WISE}{Wide-field Infrared Survey Explorer (WISE) from the IPAC All-Sky Data Release}
\newcommand{\CASA}{Common Astronomy Software Applications (CASA)}
\newcommand{\ALMA}{Atacama Large Millimeter/submillimeter Array (ALMA)}
\newcommand{\fdf}{\textit{F}$(\phi)$}
\newcommand{\I}{\textit{I}}
\newcommand{\Q}{\textit{Q}}
\newcommand{\U}{\textit{U}}
\newcommand{\Pol}{\textit{P}}
\newcommand{\QU}{\textit{QU}}
\newcommand{\ASKAP}{Australian Square Kilometre Array Pathfinder (ASKAP)}
\newcommand{\POSSUM}{Polarisation Sky Survey of the Universe's Magnetism (POSSUM)}
\newcommand{\EMU}{Evolutionary Map of the Universe (EMU)}
\newcommand{\thetaP}{$\theta_{\textrm{{\scriptsize peak}}}$}
\newcommand{\maxL}{ $\mathscr{L}_{\textrm{{\scriptsize max}}}$}
\newcommand{\chilam}{$\chi(\lambda^{2})$}
\newcommand{\Alfven}{Alfv\'{e}n }
\newcommand{\Alfvenic}{Alfv\'{e}nic }
%\newcommand{\etal}{et~al.~}
%\newcommand{\Order}{\mbox{$\mathcal{O}$}}
%
%\newcommand{\V}[1]{\mathbf{#1}} 
%%
%% reference callout
%%
%%\newcommand{\eqref}[1]{(\ref{#1})}
%\newcommand{\figref}[1]{Figure~\ref{#1}}
%\newcommand{\secref}[1]{Section~\ref{#1}}
%\newcommand{\appref}[1]{Appendix~\ref{#1}}
%\newcommand{\chapref}[1]{Chapter~\ref{#1}}
%\newcommand{\tabref}[1]{Table~\ref{#1}}
%
%\newcommand{\bhat}{\mbox{$\hat{\mathbf{b}}$}} 
%\newcommand{\zhat}{\mbox{$\hat{\mathbf{z}}$}} 
%\newcommand{\xhat}{\mbox{$\hat{\mathbf{x}}$}} 
%\newcommand{\yhat}{\mbox{$\hat{\mathbf{y}}$}} 
\newcommand{\strom}{Str\"{o}mgren }
\newcommand{\hi}{H\,{\sc i} } % HI
\newcommand{\HII}{H\,{\sc ii} } %HII region
%\newcommandd{\HII}{H{\scriptsize ii}}
%\newcommand{\farcm}{\mbox{\ensuremath{.\mkern-4mu^\prime}}}%   %fraction acrminute symbol: 0.''0
%\newcommand{\farcs}{\mbox{\ensuremath{.\!\!^{\prime\prime}}}} % fractional arcsecond symbol: 0.'0
%\newcommand{\fdg}{\mbox{\ensuremath{.\!\!^\circ}}} % fraction degree symbol
\newcommand{\ddeg}{\ensuremath{^{\circ}}} % degree symbol
%\newcommand{\farcs}{$''$}
%\newcommand{\hi}{HI }
%\newcommand{\HII}{HII }
\newcommand{\lsi}{LSI +61\ddeg303}
\newcommand{\sunn}{\ensuremath{\odot}}% sun symbol
\newcommand{\Msun}{\ensuremath{\textrm{M}_{\odot} }} % M.sun
\newcommand{\MLu}{\textrm{M}$_{\odot}$ yr$^{-1}$}
\newcommand{\kms}{km s$^{-1}$}
\newcommand{\infinity}{\ensuremath{\infty}}
\newcommand{\ML}{\ensuremath{\dot{M}}} %Mass loss rate
\newcommand{\Lsunn}{\ensuremath{L_{\odot}}}  %L.sun symbol
\newcommand{\radm}{rad m$^{-2}$}
\newcommand{\MLM}{\dot{M}}
\newcommand{\blos}{B$_{\textrm{LOS}}$}
\newcommand{\cm}{cm$^{-3}$}
\newcommand{\plam}{\textit{P($\lambda^2$)}}
\newcommand{\fsimp}{\textit{Faraday simple}}
\newcommand{\fcomp}{\textit{Faraday complex}}
\newcommand{\fphi}{\textit{F($\phi$)}}
\newcommand{\lamsq}{$\lambda^2$}
\newcommand{\rmclean}{\textsc{rmclean}}
\newcommand{\clean}{\textsc{clean}}
\newcommand{\immath}{\textsc{immath}}
\newcommand{\polcal}{\textsc{polcal}}
\newcommand{\equa}[1]{Equation (\ref{eq:#1})}
\newcommand{\equas}[2]{Equations (\ref{eq:#1}) and (\ref{eq:#2})}
\newcommand{\about}{$\sim$}
\newcommand{\mircon}{$\mu$m}

%\newcommand{\chilam}{$\chi$($\lambda^{2}$)}

%\newcommand{\Teff}{\ensuremath{T_{\mathrm{eff}}}}%              % T_eff
%\newcommand{\logg}{\ensuremath{\log g}}%                        % log g
%\newcommand{\bv}{\ensuremath{B\!-\!V}}%                         % B-V
%\newcommand{\ub}{\ensuremath{U\!-\!B}}%                         % U-B
%\newcommand{\vr}{\ensuremath{V\!-\!R}}%                         % V-R
%\newcommand{\ur}{\ensuremath{U\!-\!R}}%                         % U-R
%\newcommand\ion[2]{#1$\;${\scshape{#2}}}%                       % ion, i.e., CII = \ion{C}{ii}
%%journal title commands
%\rmfamily

%\def\ref@jnl#1{{\jnl@style#1}}%

%\begin{comment}
%\newcommand\aj{\rmfamily{AJ}}%
%%          % Astronomical Journal
%\newcommand\actaa{\rmfamily{Acta Astron.}}%
%%  % Acta Astronomica
%\newcommand\araa{\rmfamily{ARA\&A}}%
%%          % Annual Review of Astron and Astrophys
%\newcommand\apj{\rmfamily{ApJ}}%
%%          % Astrophysical Journal
%\newcommand\apjl{\rmfamily{ApJ}}%
%%          % Astrophysical Journal, Letters
%\newcommand\apjs{\rmfamily{ApJS}}%
%%          % Astrophysical Journal, Supplement
%\newcommand\ao{\rmfamily{Appl.~Opt.}}%
%%          % Applied Optics
%\newcommand\apss{\rmfamily{Ap\&SS}}%
%%          % Astrophysics and Space Science
%\newcommand\aap{\rmfamily{A\&A}}%
%%          % Astronomy and Astrophysics
%\newcommand\aapr{\rmfamily{A\&A~Rev.}}%
%%          % Astronomy and Astrophysics Reviews
%\newcommand\aaps{\rmfamily{A\&AS}}%
%%          % Astronomy and Astrophysics, Supplement
%\newcommand\azh{\rmfamily{AZh}}%
%%          % Astronomicheskii Zhurnal
%\newcommand\baas{\rmfamily{BAAS}}%
%%          % Bulletin of the AAS
%\newcommand\caa{\rmfamily{Chinese Astron. Astrophys.}}%
%%  % Chinese Astronomy and Astrophysics
%\newcommand\cjaa{\rmfamily{Chinese J. Astron. Astrophys.}}%
%%  % Chinese Journal of Astronomy and Astrophysics
%\newcommand\icarus{\rmfamily{Icarus}}%
%%  % Icarus
%\newcommand\jcap{\rmfamily{J. Cosmology Astropart. Phys.}}%
%%  % Journal of Cosmology and Astroparticle Physics
%\newcommand\jrasc{\rmfamily{JRASC}}%
%%          % Journal of the RAS of Canada
%\newcommand\memras{\rmfamily{MmRAS}}%
%          % Memoirs of the RAS
%\newcommand\mnras{\rmfamily{MNRAS}}%
%%          % Monthly Notices of the RAS
%\newcommand\na{\rmfamily{New A}}%
%%  % New Astronomy
%\newcommand\nar{\ref@jnl{New A Rev.}}%
%%  % New Astronomy Review
%\newcommand\pra{\rmfamily{Phys.~Rev.~A}}%
%%          % Physical Review A: General Physics
%\newcommand\prb{\rmfamily{Phys.~Rev.~B}}%
%%          % Physical Review B: Solid State
%\newcommand\prc{\rmfamily{Phys.~Rev.~C}}%
%%          % Physical Review C
%\newcommand\prd{\rmfamily{Phys.~Rev.~D}}%
%%          % Physical Review D
%\newcommand\pre{\rmfamily{Phys.~Rev.~E}}%
%%          % Physical Review E
%\newcommand\prl{\rmfamily{Phys.~Rev.~Lett.}}%
%%          % Physical Review Letters
%\newcommand\pasa{\rmfamily{PASA}}%
%%  % Publications of the Astron. Soc. of Australia
%\newcommand\pasp{\rmfamily{PASP}}%
%%          % Publications of the ASP
%\newcommand\pasj{\rmfamily{PASJ}}%
%%          % Publications of the ASJ
%\newcommand\qjras{\rmfamily{QJRAS}}%
%%          % Quarterly Journal of the RAS
%\newcommand\rmxaa{\rmfamily{Rev. Mexicana Astron. Astrofis.}}%
%%  % Revista Mexicana de Astronomia y Astrofisica
%\newcommand\skytel{\rmfamily{S\&T}}%
%%          % Sky and Telescope
%\newcommand\solphys{\rmfamily{Sol.~Phys.}}%
%%          % Solar Physics
%\newcommand\sovast{\rmfamily{Soviet~Ast.}}%
%%          % Soviet Astronomy
%\newcommand\ssr{\rmfamily{Space~Sci.~Rev.}}%
%%          % Space Science Reviews
%\newcommand\zap{\rmfamily{ZAp}}%
%%          % Zeitschrift fuer Astrophysik
%\newcommand\nat{\rmfamily{Nature}}%
%%          % Nature
%\newcommand\iaucirc{\rmfamily{IAU~Circ.}}%
%%          % IAU Cirulars
%\newcommand\aplett{\rmfamily{Astrophys.~Lett.}}%
%%          % Astrophysics Letters and Communications
%\newcommand\apspr{\rmfamily{Astrophys.~Space~Phys.~Res.}}%
%%          % Astrophysics Space Physics Research
%\newcommand\bain{\rmfamily{Bull.~Astron.~Inst.~Netherlands}}%
%%          % Bulletin Astronomical Institute of the Netherlands
%\newcommand\fcp{\rmfamily{Fund.~Cosmic~Phys.}}%
%          % Fundamental Cosmic Physics
%\newcommand\gca{\rmfamily{Geochim.~Cosmochim.~Acta}}%
%%          % Geochimica Cosmochimica Acta
%\newcommand\grl{\rmfamily{Geophys.~Res.~Lett.}}%
%%          % Geophysics Research Letters
%\newcommand\jcp{\rmfamily{J.~Chem.~Phys.}}%
%%          % Journal of Chemical Physics
%\newcommand\jgr{\rmfamily{J.~Geophys.~Res.}}%
%%          % Journal of Geophysical Research
%\newcommand\jqsrt{\rmfamily{J.~Quant.~Spec.~Radiat.~Transf.}}%
%%          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
%\newcommand\memsai{\rmfamily{Mem.~Soc.~Astron.~Italiana}}%
%%          % Mem. Societa Astronomica Italiana
%\newcommand\nphysa{\rmfamily{Nucl.~Phys.~A}}%
%%          % Nuclear Physics A
%\newcommand\physrep{\rmfamily{Phys.~Rep.}}%
%%          % Physics Reports
%\newcommand\physscr{\rmfamily{Phys.~Scr}}%
%%          % Physica Scripta
%\newcommand\planss{\rmfamily{Planet.~Space~Sci.}}%
%%          % Planetary Space Science
%\newcommand\procspie{\rmfamily{Proc.~SPIE}}%
%%          % Proceedings of the SPIE
%\let\astap=\aap
%\let\apjlett=\apjl
%\let\apjsupp=\apjs
%\let\applopt=\ao
%\end{comment}
